AnthroNet: Conditional Generation of Humans via Anthropometrics

We present a novel human body model formulated by an extensive set of anthropocentric measurements, which is capable of generating a wide range of human body shapes and poses. The proposed model enables direct modeling of specific human identities through a deep generative architecture, which can produce humans in any arbitrary pose. It is the first of its kind to have been trained end-to-end using only synthetically generated data, which not only provides highly accurate human mesh representations but also allows for precise anthropometry of the body. Moreover, using a highly diverse animation library, we articulated our synthetic humans' body and hands to maximize the diversity of the learnable priors for model training. Our model was trained on a dataset of $100k$ procedurally-generated posed human meshes and their corresponding anthropometric measurements. Our synthetic data generator can be used to generate millions of unique human identities and poses for non-commercial academic research purposes.

==> 05_05_anthro_regressor.tex <==

% \begin{figure}[!htb]
%   \centering
%   \begin{subfigure}[t]{\linewidth}
%       \includegraphics[width=\linewidth, trim={17cm 18cm 4cm 16cm}, clip]{figs_pdf_300dpi/masks/soft_mask_Male_left_calf_length.png}
%       \caption{Left calf length male mask}
%         \label{fig:buffers-mask}
%     \end{subfigure}
%     \hspace{1.5em}
%     \begin{subfigure}[t]{\linewidth}
% \includegraphics[width=\linewidth, trim={17cm 18cm 4cm 16cm}, clip]{figs_pdf_300dpi/masks/soft_mask_Female_hip_circumference.png}
%         \caption{Hip circumference female mask}
%         \label{fig:buffers-nopb}
%     \end{subfigure}
%   \caption{\todo{figure needs to go to appendix. It is very hard to interpret, as it is small and uses a bad colormap} After isolating the mesh related volume, we calculated the minimal Euclidian distance \begin{math}d_{min}\end{math} between each vertices of the volume and the ones used for the anthropometric measure. The final weight in the mask associated to the vertex point is \begin{math}e^{d_{min}}\end{math}. 
% }
%   \label{fig:masks}
% \end{figure}

% In order to facilitate the evaluation of our model on the Humans in the Wild dataset~\cite{Shapy:CVPR:2022}, we trained a regression model that extracts the anthropometric measurements from registered meshes. 
% During each optimization step of the registration pipeline, a T-pose mesh is generated by the model presented in sec.~\ref{subsec:mesh_gen}. We then use the anthropometric regressor model to provide us with the estimated body measurements on the produced mesh. Lastly, the rigging and skinning model adjust the mesh to the desired pose. 

% For each of the 36 anthropometric measurements defined in sec.~\ref{subsec:anthro}, we trained an expert Multi Layer Perceptron~\cite{haykin1994neural} comprised of three layers. To ensure the disentanglement between the anthropometric measures, we designed a mask for each measure to isolate the vertices on the mesh related to the measure as shown in fig.~\ref{fig:masks}. This design prevents interference from other vertices in the prediction of a measure on a specific body part. 
% % During training, the input is the masked mesh where the mesh is multiplied by the mask as you can see in Figure \ref{fig:masks}. 
% % At inference time, the input is still a mesh and we are collecting the output of all the 36 models and aggregating the results. 


==> supp_mat_main.tex <==
% % \section{Appendix}
% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%% PAPER TYPE  - PLEASE UPDATE FOR FINAL VERSION %%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \usepackage[review]{cvpr}      % To produce the REVIEW version
% % \usepackage{cvpr}              % To produce the CAMERA-READY version
% \usepackage[pagenumbers]{cvpr} % To force page numbers, e.g. for an arXiv version


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  STANDARD PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage{csvsimple}
% \usepackage[shortlabels]{enumitem}
% % \usepackage[numbers,sort,compress]{natbib} % for other bib styles


% % It is strongly recommended to use hyperref, especially for the review version.
% % hyperref with option pagebackref eases the reviewers' job.
% % Please disable hyperref *only* if you encounter grave issues, e.g. with the
% % file validation for the camera-ready version.
% %
% % If you comment hyperref and then uncomment it, you should deletehttps://www.overleaf.com/project/6310e6316c5fb422272532ef
% % ReviewTempalte.aux before re-running LaTeX.
% % (Or just hit 'q' on the first LaTeX run, let it finish, and you
% %  should be clear).
% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}


% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% USER PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \usepackage{subfig} % outdated, use subcaption instead
% % \usepackage{rotating}
% % \usepackage{subcaption} %to have subfigures available
% % \usepackage{adjustbox}
% % \usepackage{float}
% \usepackage{multirow}
% % \usepackage[compact]{titlesec}
% % \usepackage[inline]{enumitem}
% % \usepackage{enumerate}
% % % \bibliographystyle{abbrvnat}
% % % \usepackage{algorithm}
% % % \usepackage{algpseudocode}
% \usepackage{xcolor}         % colors
% \usepackage{dsfont}
% \usepackage{mathrsfs}
% \usepackage[group-separator={,}]{siunitx}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%% TAG YOUR CO-AUTHORS LIKE SO %%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newcommand{\todo}[1]{{\color{red}{}#1}}
% \newcommand{\sujoy}[1]{{\color{magenta}{\bf Sujoy: }#1}}
% \newcommand{\francesco}[1]{{\color{violet}{\bf Francesco: }#1}}
% \newcommand{\salehe}[1]{{\color{cyan}{\bf Salehe: }#1}}
% \newcommand{\shrinath}[1]{{\color{teal}{\bf Shrinath: }#1}}
% \newcommand{\soroosh}[1]{{\color{orange}{\bf Soroosh: }#1}}
% \newcommand{\jonathan}[1]{{\color{pink}{\bf Jonathan: }#1}}
% \newcommand{\jay}[1]{{\color{purple}{\bf Jay: }#1}}
% \newcommand{\peifeng}[1]{{\color{brown}{\bf Peifeng: }#1}}
% \newcommand{\david}[1]{{\color{olive}{\bf David: }#1}}
% \newcommand{\charles}[1]{{\color{green}{\bf Charles: }#1}}
% \newcommand{\mesh}{$\mathcal{X}^A_b$}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PAPER ID  - 6070 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \def\cvprPaperID{6070} % Salehe's submission
% \def\cvprPaperID{11852} % Francesco's submission - possibly go with this if Salehe is traveling and can't make the supplementary material submission by Nov 18
% \def\confName{CVPR}
% \def\confYear{2023}
% \def\proposed{AnthroNet }

% \begin{document}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TITLE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \title{One Model to Represent Them All, and in the Hidden Space Bind Them}
% \title{Appendix - AnthroNet: Conditional Generation of Humans via Anthropometrics}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%% AUTHOR LIST - USE THIS %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \author{Francesco Picetti$^*$
% \quad
% Shrinath Deshpande$^*$
% \quad
% Jonathan Leban$^*$
% \quad
% Soroosh Shahtalebi$^\dagger$
% \quad
% Jay Patel$^\dagger$
% \\
% Peifeng Jing
% \quad
% Chunpu Wang
% \quad
% Charles Metze III
% \quad
% Sujoy Ganguly$^\S$
% \quad
% Salehe Erfanian Ebadi$^\S$
% \vspace{0.2cm}
% \\
% \vspace{0.1cm}
% \textbf{Unity Technologies}\\
% {
% \tt\small
% \{francesco.picetti,
% shrinath.deshpande, 
% jonathan.leban, 
% soroosh.shahtalebi, 
% jay.patel, 
% \\
% \tt\small 
% peifeng.jing, 
% davidwang, 
% charles.metze, 
% sujoy.ganguly, 
% salehe.erfanianebadi\}@unity3d.com
% }
% }

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%% CVPR AUTHOR LIST - DO NOT USE - THIS FORMAT WASTES SPACE %%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \author{Francesco Picetti$^*$
% % % Unity Technologies\\
% % % {\tt\small francesco.picetti@unity3d.com}
% % \and
% % Shrinath Deshpande$^*$
% % % Unity Technologies\\
% % % {\tt\small shrinath.deshpande@unity3d.com}
% % \and
% % Jonathan Leban$^*$
% % % Unity Technologies\\
% % % {\tt\small jonathan.leban@unity3d.com}
% % \and
% % Soroosh Shahtalebi$^\dagger$
% % % Unity Technologies\\
% % % {\tt\small soroosh.shahtalebi@unity3d.com}
% % \and
% % Jay Patel$^\dagger$
% % % Unity Technologies\\
% % % {\tt\small jay.patel@unity3d.com}
% % \and
% % Peifeng Jing
% % % Unity Technologies\\
% % % {\tt\small peifeng.jing@unity3d.com}
% % \and
% % Chunpu Wang
% % % Unity Technologies\\
% % % {\tt\small davidwang@unity3d.com}
% % \and
% % Charles Metze III
% % % Unity Technologies\\
% % % {\tt\small charles.metze@unity3d.com}
% % \and
% % Sujoy Ganguly$^\S$
% % % Unity Technologies\\
% % % {\tt\small sujoy.ganguly@unity3d.com}
% % \and
% % Salehe Erfanian Ebadi$^\S$
% % % Unity Technologies\\
% % % {\tt\small salehe.erfanianebadi@unity3d.com}
% % % \\
% % }

% \maketitle

% \appendix

% \section{Design Parameters}\label{supp:design_parameters}
% This section provides a description of all the deep neural networks and the details of the anthropometric measurements introduced in this work.
% \input{09_01_mesh_gen_arch}


% \input{09_02_anthro_measures_details}

% \input{09_03_anthro_regressor}

% \input{09_04_mesh_skinner_rigger_arch}


% \input{09_05_registration_pipeline}

% \section{Extended Experiments and Results}\label{supp:extended_experiments}

% \input{09_06_extended_results}

% \input{09_07_B2A}

% {\small
% \bibliographystyle{ieee_fullname} % orig
% % \bibliographystyle{abbrvnat}
% % \bibliographystyle{abbrv}
% \bibliography{egbib}
% }


% \end{document}

==> tables/generative_model_ablations.tex <==
\begin{tabular}{lllllll}
\toprule
      model\_name &             run\_name & epoch &         huber\_loss\_val &                                conditional\_columns & loader/batch\_size & model/args/fourier\_dim \\
\midrule
            CVAE &                 cvae & 200.0 &  1.545140185044147e-05 &                      height\_param,weight\_param,sex &                32 &                    NaN \\
ECVAE\_Conditions & ecvae 16 frequencies &  13.0 & 2.9062110115773976e-05 &                                anthropometrics,sex &               128 &                     16 \\
ECVAE\_Conditions & ecvae 32 frequencies &  13.0 & 4.2586576455505565e-05 &                                anthropometrics,sex &               128 &                     32 \\
            CVAE &          vae-vanilla &  44.0 &  5.011134271626361e-05 & waist\_circumference,chest\_circumference,hip\_cir... &                32 &                    NaN \\
            CVAE &             cvae-few & 200.0 &  5.013536065234803e-05 & waist\_circumference,chest\_circumference,hip\_cir... &               128 &                    NaN \\
ECVAE\_Conditions & ecvae 16 frequencies & 107.0 &  5.802185569336871e-06 &                                anthropometrics,sex &               128 &                     16 \\
ECVAE\_Conditions &   ecvae no laplacian & 200.0 &  7.000391178735299e-06 &                                anthropometrics,sex &                32 &                      8 \\
            CVAE &         cvae default & 110.0 &  7.347938208113192e-06 &                                anthropometrics,sex &               128 &                    NaN \\
            CVAE &          vae-vanilla &  53.0 &   9.40214977163123e-06 &                      height\_param,weight\_param,sex &                32 &                    NaN \\
            CVAE &           cvae shapy & 109.0 &   9.74598660832271e-05 & height,waist\_circumference,chest\_circumference,... &               128 &                    NaN \\
ECVAE\_Conditions &   ecvae default 100k & 200.0 &  9.888291060633492e-06 &                                anthropometrics,sex &                32 &                      8 \\
\bottomrule
\end{tabular}
